MetaTra: Meta-Learning for Generalized Trajectory Prediction in Unseen Domain

Trajectory prediction has garnered widespread attention in different fields, such as autonomous driving and robotic navigation. However, due to the significant variations in trajectory patterns across different scenarios, models trained in known environments often falter in unseen ones. To learn a generalized model that can directly handle unseen domains without requiring any model updating, we propose a novel meta-learning-based trajectory prediction method called MetaTra. This approach incorporates a Dual Trajectory Transformer (Dual-TT), which enables a thorough exploration of the individual intention and the interactions within group motion patterns in diverse scenarios. Building on this, we propose a meta-learning framework to simulate the generalization process between source and target domains. Furthermore, to enhance the stability of our prediction outcomes, we propose a Serial and Parallel Training (SPT) strategy along with a feature augmentation method named MetaMix. Experimental results on several real-world datasets confirm that MetaTra not only surpasses other state-of-the-art methods but also exhibits plug-and-play capabilities, particularly in the realm of domain generalization.

==> figs/ETH-UCY-STATICS.tex <==
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \includegraphics[width=1\linewidth]{figs/figs/ETH-UCY statics.png} % 请确保文件路径和文件名正确
    \caption{Density, Speed, and Acceleration in ETH-UCY Dataset}
    \label{fig:ETH-UCY-statics}
\end{figure}


==> figs/SDD-split.tex <==
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \includegraphics[width=1\linewidth]{figs//figs/SDD-SPLIT.png} % 请确保文件路径和文件名正确
    \caption{Performance comparison of eight SDD scenarios. With MGTP, the performance rises are significant. }
    \label{fig:SDD-split}
\vspace{-0.5cm}
\end{figure}


==> figs/SDD_radar.tex <==
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \begin{subfigure}{0.225\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/AN-AV.png}
        \caption{Density and Speed }
        \label{fig:AN-AV}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.225\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/AA.png}
        \caption{Acceleration}
        \label{fig:AA}
    \end{subfigure}
    \caption{Statistics of eight scenes}
    \label{fig:SDD_radar}
\end{figure}

==> figs/SNE3.tex <==
\begin{figure*}[htpb]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/ETH-UCY statics.png} 
        \caption{Density(AN),Speed(AV),and Acceleration(AA) in ETH-UCY Dataset }
        \label{fig:ETH-UCY-statics}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/eth52sne.png}
        \caption{ HSTTE }
        \label{fig:HSTTE}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/eth299snetry1.png}
        \caption{HSTTE + MGTP}
        \label{fig:HSTTE+ MGTP}
    \end{subfigure}
    \caption{Visualization of the domain generalization embedding learning results using t-SNE}
    \label{fig:SDD_detail_analysis3}
\vspace{-0.5cm}
\end{figure*}

==> figs/traj_vis.tex <==
\begin{figure}[htbp]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/gatesppt.png}
        \caption{\text{Gates}}
        \label{fig:Gates}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/littleppt.png}
        \caption{\text{Little}}
        \label{fig:Little}
    \end{subfigure}
        \hfill
    \begin{subfigure}{0.15\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/figs/nexusppt.png}
        \caption{\text{Nexus}}
        \label{fig:Nexus}
    \end{subfigure}
    \caption{Trajectory visualization of 3 scenes in SDD}
    \label{fig:Trajectory visualization}
\vspace{-0.5cm}
\end{figure}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/AblationMAMLMVMIX.tex <==
\begin{table*}[htpb]
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{-0.2cm}
    \centering
    \caption{Ablation studies of different meta-learning modules on the ETH-UCY dataset. We report \text{minADE$_{20}$}/\text{minFDE$_{20}$} (meters).}
    \label{tab:Ablation}
    \resizebox{1.0\textwidth}{!}
    {
    \begin{tabular}{c c c c |c c c c c |c}
        \hline
        MAML & MLDG & MVDG & MIXUP & ETH & HOTEL & UNIV & ZARA1 & ZARA2 & AVG \\
        \hline
        $\times$ & $\times$ & $\times$ & $\times$             & 0.289/0.544 & 0.153/0.281 & 0.315/0.612 & 0.233/0.475 & 0.188/0.378 & 0.2356/0.4580 \\
        $\checkmark$ & $\times$ & $\times$ & $\times$         & 0.279/0.536 & 0.147/0.280 & 0.305/0.606 & 0.243/0.524 & 0.184/0.380 & 0.2288/0.4532 \\
        $\times$ & $\checkmark$ & $\times$ & $\times$         & 0.271/0.512 & 0.136/0.249 & 0.295/0.590 & 0.195/0.412 & 0.177/0.369 & 0.2148/0.4264 \\
        $\times$ & $\checkmark$ & $\checkmark$ & $\times$     & 0.258/0.491 & 0.130/0.240 & 0.292/0.586 & 0.187/0.396 & 0.166/0.343 & 0.2066/0.4112 \\
        $\times$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 0.245/0.465 & 0.130/0.233 & 0.290/0.586 & 0.184/0.392 & 0.162/0.332 & 0.2034/0.4034 \\
        \hline
    \end{tabular}
    }
\end{table*}



==> tables/tables.tex <==
\begin{table*}[htpb]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\caption{\text{minADE$_{20}$}/\text{minFDE$_{20}$} (meters) of trajectory prediction (ETH-UCY dataset).
%``AVG" represents the average results across the five scenarios in ETH-UCY). \textbf{Bold}/\underline{underlined} fonts represent the best/second-best result.
$^*$ denotes that Agent Former is the previous best model on this dataset. With MVL, Agent Former works even better. Our backbone Dual-TT with MGTP achieves achieves comparable results.}
\label{tab:ETH-UCY}
\resizebox{1.0\textwidth}{!}
{
\begin{tabular}{|l|c c c c c|c c|c c|}
\hline
\multirow{2}{*}{Subset} & Social-STGCNN & Trajectron++ & PECNet & STAR & GroupNet & Agent Former$^*$ & Agent Former$^*$ & Dual-TT & Dual-TT\\
& \textcolor{blue}{CVPR20\cite{Social-STGCNN}} & \textcolor{blue}{ECCV20\cite{Trajectron++}} & \textcolor{blue}{ECCV20\cite{PecNet}} & \textcolor{blue}{ECCV20\cite{STAR}} & \textcolor{blue}{CVPR22\cite{groupnet}} & \textcolor{blue}{ICCV21\cite{AgentFormer}} & +MGTP &  & + MGTP\\
\hline
ETH & 0.64/1.11 & 0.61/1.02 & 0.54/0.87 & 0.36/0.65 & 0.46/0.73 & 0.45/0.75 & 0.36/0.57 & \underline{0.29/0.54} & \textbf{0.24/0.46} \\
HOTEL & 0.49/0.85 & 0.19/0.28 & 0.18/0.24 & 0.21/0.41 & 0.15/0.25 & 0.14/0.22 & \textbf{0.13/0.21} & 0.15/0.28 & \underline{0.13/0.23} \\
UNIV & 0.44/0.79 & 0.30/0.54 & 0.35/0.60 & 0.33/0.67 & 0.26/0.45 & \underline{0.25/0.45} & \textbf{0.24/0.43} & 0.31/0.61 & 0.29/0.58 \\
ZARA1 & 0.34/0.53 & 0.24/0.42 & 0.22/0.39 & 0.29/0.52 & 0.21/0.39 & \textbf{0.18/0.30} & 0.19/0.30 & 0.23/0.46 & \underline{0.18/0.39} \\
ZARA2 & 0.30/0.48 & 0.18/0.32 & 0.17/0.30 & 0.22/0.46 & 0.17/0.33 & \underline{0.14/0.24} & \textbf{0.13/0.22} & 0.19/0.38 & 0.16/0.33 \\
AVG & 0.44/0.75 & 0.30/0.51 & 0.29/0.48 & 0.28/0.54 & 0.25/0.44 & 0.23/0.39 & \underline{0.21/0.35} & 0.23/0.45 & \textbf{0.20/0.40} \\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[htpb]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\caption{\text{minADE$_{20}$} / \text{minFDE$_{20}$} (pixels) of trajectory prediction (SDD dataset).
%\textbf{Bold}/\underline{underlined} fonts represent the best/second-best result. 
$^*$ denotes that PECNet is the previous best model on this dataset. With MGTP, PECNet works even better. Our backbone Dual-TT with MGTP achieves the current best ADE result.}
\label{tab:SDD}
\resizebox{1.0\textwidth}{!}
{
\begin{tabular}{|l|c c c c c |c c|c c|}
\hline
\multirow{2}{*}{agents type} & Social-STGCNN & Trajectron++ & STAR  & Agent Former & Group Net & PECNet$^*$ & PECNet$^*$ & Dual-TT & Dual-TT\\
& \textcolor{blue}{CVPR20\cite{Social-STGCNN}} & \textcolor{blue}{ECCV20\cite{Trajectron++}} & \textcolor{blue}{ECCV20\cite{STAR}} & \textcolor{blue}{ICCV21\cite{AgentFormer}} & \textcolor{blue}{CVPR22\cite{groupnet}} & \textcolor{blue}{ECCV20\cite{PecNet}} & + MGTP &  & +MGTP\\
\hline
pedestrian & 20.25/35.75  & 19.30/32.70 & 17.63/36.21 & 10.32/18.30%参考自DynGroupNet
& 9.31/16.11  & 9.96/15.88  & \underline{8.91/13.38} & 12.79/15.88 & \textbf{8.49/11.85}  \\
all-agents     & 27.23/41.44%参考自P2T 
&  25.66/39.76  & 27.73/52.37 & 16.84/29.82 & 14.05/27.67 & 14.18/24.47 & \underline{10.97/18.40} & 16.27/29.38 & \textbf{10.13/17.05} \\
\hline
\end{tabular}
}
\vspace{-0.5cm}
\end{table*}

\begin{table*}[h]
\setlength{\abovecaptionskip}{0cm}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\caption{\text{minADE$_{20}$} / \text{minFDE$_{20}$}(meters) of trajectory prediction (NBA dataset).
%\textbf{Bold}/\underline{underlined} fonts represent the best/second-best result.
$^*$ denotes that GroupNet is the previous best model on this dataset. With MGTP, GroupNet works even much better. Our backbone Dual-TT with MGTP achieves the current best result.}
\label{tab:NBA}
\resizebox{1.0\textwidth}{!}
{
\begin{tabular}{|l|c c c c c |c c|c c|}
\hline
\multirow{2}{*}{agents type} & Social-STGCNN & Trajectron++ & Agent Former &STAR & PECNet  & GroupNet$^*$ & GroupNet$^*$ & Dual-TT & Dual-TT\\
& \textcolor{blue}{CVPR20\cite{Social-STGCNN}} & \textcolor{blue}{ECCV20\cite{Trajectron++}} & \textcolor{blue}{ICCV21\cite{AgentFormer}} & \textcolor{blue}{ECCV20\cite{STAR}} & \textcolor{blue}{ECCV20\cite{PecNet}} & \textcolor{blue}{CVPR22\cite{groupnet}} & +MGTP &   & +MGTP\\
\hline
1.0s & 0.41/0.62 & 0.30/0.38 & 0.45/0.64 & 0.43/0.66 & 0.40/0.71 & 0.26/0.34 & \underline{0.25/0.32} & 0.26/0.39 & \textbf{0.23/0.35} \\
2.0s & 0.81/1.32 & 0.59/0.82 & 0.84/1.44 & 0.75/1.24 & 0.83/1.61 & 0.49/0.70 & 0.46/0.66 & \underline{0.44/0.71} & \textbf{0.42/0.60} \\
3.0s & 1.19/1.94 & 0.85/1.24 & 1.24/2.18 & 1.03/1.51 & 1.27/2.44 & 0.73/1.02 & 0.70/0.97 & \underline{0.67/1.23} & \textbf{0.64/0.92} \\
4.0s & 1.59/2.41 & 1.15/1.57 & 1.62/2.84 & 1.13/2.01 & 1.69/2.95 & 0.96/1.30 & 0.93/1.21 & \underline{0.87/1.45} & \textbf{0.82/1.37} \\
\hline
\end{tabular}
}
\vspace{-0.3cm}
\end{table*}
